SENet: Visual Detection of Online Social Engineering Attack Campaigns

Social engineering (SE) aims at deceiving users into performing actions that may compromise their security and privacy. These threats exploit weaknesses in human's decision making processes by using tactics such as pretext, baiting, impersonation, etc. On the web, SE attacks include attack classes such as scareware, tech support scams, survey scams, sweepstakes, etc., which can result in sensitive data leaks, malware infections, and monetary loss. For instance, US consumers lose billions of dollars annually due to various SE attacks. Unfortunately, generic social engineering attacks remain understudied, compared to other important threats, such as software vulnerabilities and exploitation, network intrusions, malicious software, and phishing. The few existing technical studies that focus on social engineering are limited in scope and mostly focus on measurements rather than developing a generic defense. To fill this gap, we present SEShield, a framework for in-browser detection of social engineering attacks. SEShield consists of three main components: (i) a custom security crawler, called SECrawler, that is dedicated to scouting the web to collect examples of in-the-wild SE attacks; (ii) SENet, a deep learning-based image classifier trained on data collected by SECrawler that aims to detect the often glaring visual traits of SE attack pages; and (iii) SEGuard, a proof-of-concept extension that embeds SENet into the web browser and enables real-time SE attack detection. We perform an extensive evaluation of our system and show that SENet is able to detect new instances of SE attacks with a detection rate of up to 99.6% at 1% false positive, thus providing an effective first defense against SE attacks on the web.

==> framework_details_current_editSK.tex <==
\section{ Framework Details Contd.}


==> references.tex <==

\begin{thebibliography}{1}


\bibitem{puppeteer}
   https://pptr.dev
\bibitem{tranco}
   https://tranco-list.eu
\bibitem{phani} 
   Vadrevu, Phani, and Roberto Perdisci. "What you see is not what you get: Discovering and tracking social engineering attack campaigns." In Proceedings of the Internet Measurement Conference, pp. 308-321. 2019.
\bibitem{karthika}
  Subramani, Karthika, Xingzi Yuan, Omid Setayeshfar, Phani Vadrevu, Kyu Hyung Lee, and Roberto Perdisci. "When push comes to ads: Measuring the rise of (malicious) push advertising." In Proceedings of the ACM Internet Measurement Conference, pp. 724-737. 2020.
\bibitem{turk}
  https://www.mturk.com
\bibitem{stealth}
 https://www.npmjs.com/package/puppeteer-extra-plugin-stealth
\bibitem{Szegedy}
  Szegedy, Christian, Sergey Ioffe, Vincent Vanhoucke, and Alexander Alemi. "Inception-v4, inception-resnet and the impact of residual connections on learning." In Proceedings of the AAAI conference on artificial intelligence, vol. 31, no. 1. 2017.
\bibitem{Kaiming}
  He, Kaiming, Xiangyu Zhang, Shaoqing Ren, and Jian Sun. "Deep residual learning for image recognition." In Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 770-778. 2016.
\bibitem{Simonyan}
   Simonyan, Karen, and Andrew Zisserman. "Very deep convolutional networks for large-scale image recognition." arXiv preprint arXiv:1409.1556 (2014).
\bibitem{Chollet}
   Chollet, François. "Xception: Deep learning with depthwise separable convolutions." In Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 1251-1258. 2017.



\bibitem{Imagenet}
Deng, Jia, Wei Dong, Richard Socher, Li-Jia Li, Kai Li, and Li Fei-Fei. "Imagenet: A large-scale hierarchical image database." In 2009 IEEE conference on computer vision and pattern recognition, pp. 248-255. Ieee, 2009.

\bibitem{Imagenetchallenge}
Russakovsky, Olga, Jia Deng, Hao Su, Jonathan Krause, Sanjeev Satheesh, Sean Ma, Zhiheng Huang et al. "Imagenet large scale visual recognition challenge." International journal of computer vision 115 (2015): 211-252.

\bibitem{determinism}
\url{https://www.tensorflow.org/api_docs/python/tf/config/experimental/enable_op_determinism}

\bibitem{Jonathan}   
  Long, Jonathan, Evan Shelhamer, and Trevor Darrell. "Fully convolutional networks for semantic segmentation." In Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 3431-3440. 2015.
\bibitem{McMahan}
  McMahan, Brendan, and Daniel Ramage. "Federated learning: Collaborative machine learning without centralized training data." Google Research Blog 3 (2017).
\bibitem{simulation}
  \url{ https://www.tensorflow.org/federated/tutorials/simulations}
\bibitem{Tajbakhsh}
  Tajbakhsh, Nima, Jae Y. Shin, Suryakanth R. Gurudu, R. Todd Hurst, Christopher B. Kendall, Michael B. Gotway, and Jianming Liang. "Convolutional neural networks for medical image analysis: Full training or fine tuning?." IEEE transactions on medical imaging 35, no. 5 (2016): 1299-1312
\bibitem{Shuicheng}
  Lin, Min, Qiang Chen, and Shuicheng Yan. "Network in network." arXiv preprint arXiv:1312.4400 (2013).
\bibitem{Micikevicius}
  Micikevicius, Paulius, Sharan Narang, Jonah Alben, Gregory Diamos, Erich Elsen, David Garcia, Boris Ginsburg et al. "Mixed precision training." arXiv preprint arXiv:1710.03740 (2017).
\end{thebibliography}


==> senet-old.tex <==
\subsection{SENet}
\label{sec:senet}
We build this research around developing SENet, a practical and deployable detection system for Social Engineering attacks. Given its importance, we attempt to explain the reasoning for various design decisions of SENet module. During design phase, We envisioned SENet to be capable of identifying web based SE Attacks tailored by adversaries to target users across a wide range of devices, including mobiles, laptops, tablets, and desktops. To that end, we identify and address the following design questions and explain the steps taken to address them as follows. 


\begin{tcolorbox}
    DQ1: What traits of SE attacks are unique enough to aid its detection?
\\   DQ2: How to make SENet adaptable in order to detect SE attacks across multiple devices?
\\  DQ3: How to implement it efficiently given limited resources? 
\end{tcolorbox}


First, regardless of the device, once a SE attack is visually rendered in a client's browser, they are known to exhibit certain visual traits that are pertinent to the attack's success. Therefore, we consider these visual cues to be reliable indicators of SE attacks that forms the basis for our decision to build a visual based detection system, {\em SENet}. In light of this, we opt to approach our attack classification task in a manner similar to an Image classification task, in turn, leading us to adopt deep learning techniques that are state-of-the-art in Image classification tasks. 

Second, it should be noted that it is not as straightforward as training traditional convolutional neural networks(CNNs) on SE screenshots to obtain the desired output. One of the benefits of deep learning techniques is that we could use transfer learning to tailor a pre-trained model to suit our current task instead of training a model from scratch thus saving more time and resources. However, some caveats exists in using such pre-trained models; Few traditional CNNs(e.g., VGG16, ResNet50, etc.), are limited by their design to accept images of fixed input size(e.g., 224x224) and fixed aspect ratio. This, in turn, limits us from designing a detection system that can handle images of arbitrary sizes with largely varying aspect ratios. Further, resizing images to fit the input size would easily distort its important features. To address this significant issue, we leverage the advantages offered by Fully Convolutional Networks(FCNs) that were proposed for image segmentation tasks. 

\noindent \textbf{FCN Benefits: } FCNs, or Fully Convolutional Networks, offer several advantages for tasks like semantic segmentation including handling images of variable sizes and faster training time. Semantic segmentation is a computer vision task that   aims to provide a detailed understanding of the image by assigning class labels to individual pixels, unlike other forms of image classification that assign a single label to the entire image. Further, FCN incorporates multiple design features that results in accurate segmentation, even after down sampling, while still preserving fine-grained details within images. These benefits prove to offer the required solution for the shortcomings of some traditional CNN network that requires images of fixed size. 

\noindent \textbf{Adopting FCN: } To convert a traditional CNN  into a Fully Convolutional Network, we included a GlobalMaxPooling2D layer after the last Conv2D layer. This additional layer takes the feature maps produced by the preceding Conv2D layer, identifies the most significant features, and applies max pooling across the entire feature map. As a result, a single value is obtained for each channel in the feature map. Finally, we included a dense layer in our binary classification task, consisting of two neurons and utilizing the Softmax activation function for classification.


\begin{algorithm}
    \caption{SENet: Custom Fully Conv. Federated Learning Training}
    \label{alg:ALG2}
    \begin{algorithmic}
    \Require {\\$SENet:$ FCN VGG19 model with Imagenet weights\\$GE:$ Global epoch count\\$CE=5:$ Client epoch count \\$CC:$ Client count,\\$SWL:$ List to store scaled client weights}
    \Ensure {A trained FCN VGG19 model}
    \\
    \end{algorithmic}
    \begin{algorithmic}[1]
    \ForAll  {$j=1$ to $GE$}
        \ForAll  {$i=1$ to $CC$}
            \State        Set $clientModel.weights = SENet.weights $ 
            \State        Create a dataset for $ith$ client by preprocessing an exact number of images from all resolutions per class
            \State        Train the client model for $CE$ epochs
            \State        Scale the weights of $clientModel$ based on $CC$
            \State        $SWL$.insert($clientModel.weights$)
        \EndFor 
        \State        Set $averageWeights$ = average weights in $SWL$
        \State        Set $SENet.weights = averagedClientWeights $ 
        \State        Evaluate $SENet$ on validation data
    \EndFor 

    \end{algorithmic}
\end{algorithm}

Third, another significant challenge is to ensure that we are able to train the customized deep learning model on large dataset of images without running into issues such as memory exhaustion as noticed during the initial experimentation stages. To overcome this challenge, we devised a customized version of the federated learning approach.

\noindent \textbf{Localized Federated Learning: }Federated learning \cite{McMahan} is a technique in machine learning where a training load can be efficiently distributed across numerous devices, whereby each device performs local training and only shares model updates with a central server. This approach could be leveraged to avoid loading an entire dataset in the memory and train individual clients on only a portion of the dataset. At the end of their training, each client would then share their results to the primary server model thus enabling effective training on large datasets. Algorithm~\ref{alg:ALG1} summarizes the multiple steps involved in training SENet that leverages FCN and Federated Learning.

==> system_details.tex <==
\section{System Details}
This section provides a detailed explanation of our system, which employs a novel approach to detect web-based social engineering attacks on the internet without compromising their aspect ratio. These attacks are similar or identical to those encountered by the model during its training. We can see a high-level representation of our system in Figure \ref{fig:fig_overview}. In the first step, we get the list of websites with low-tier ad networks prone to utilizing social engineering techniques and a set of popular benign websites. In the second step, we supply those URLs to containerized puppeteer \cite{puppeteer} crawlers. After we crawl all these URLs and collect various data, we extract the screenshots from them in step 3. Next, we processed and labeled those screenshots at step 4 to prepare them for the deep learning pipeline. After this step, we obtain what we call single-image datasets for 2 different classes, namely benign and malicious. Furthermore, we created a combined dataset by pairing screenshots in the order visited by our crawler. Then at the deep learning part, we supplied those datasets to our custom fully convolutional federated model and initialized the training loop.

% \karthika{A very brief introduction of the whole system pipeline and explain each component in detail}

\subsection{\textbf{Data Collection and Processing}}
In this section, we will give the details of dataset collection and preparation for the deep learning pipeline.


\subsubsection{\textbf{Finding Seed URLs}}
The first step is finding the seed URLs for benign and social engineering crawlers. We got the list of the most popular 5000 websites for benign crawlers from Tranco's ranking list \cite{tranco}. For the SE URLs list, we used the same approach to \cite{phani}\cite{karthika} and searched for low-tier advertisement networks that are likely to advertise such social engineering campaigns. After getting a list of such low-tier ad networks, we utilized the publicwww.com inverse code search engine to find the publisher websites to crawl. 


\begin{figure*}[ht]
    \centering
    \begin{center}
        % \vspace{18pt}%
        % \caption@setup{format=plain,justification=centering}
        \includegraphics[width=18cm,keepaspectratio]{figures/figure1_system_overview.pdf}
        
        \caption{System Overview}
        \label{fig:fig_overview}
    \end{center}

\end{figure*}


\subsubsection{\textbf{Running Benign and SE Crawlers}}
We developed a crawler application using Node.js puppeteer on the latest version of Chrome to crawl collected benign and SE URLs lists. Our crawler works pretty similarly to the crawler in \cite{phani}. The difference in our version lies in the logs we collected, the modifications to the clicking mechanism, and the addition of new emulated devices and aspect ratios/viewport sizes. In addition to taking screenshots of the visited webpages, our crawler saves the HTML composition of the webpages in MHTML format, all the request-response pairs and browser console logs, and all the downloaded files. When our automated browser performs emulated clicks on desktop devices or emulated taps on mobile devices, in addition to clicking on the images and iframes after ordering them by size related to the rendering area, we generate a static list of keywords common among social engineering examples. Some of those keywords are: "next, update, install, download, play, coupon, claim." Our crawler finds the coordinates of those elements and keywords, performs several clicks defined as a parameter, visits the new tabs opened by those clicks, and performs the same on those tabs and saves that information along with the order of the URLs by visit timestamp to the "Traceback Logs" file in JSON format. Because social engineering attacks vary in design depending on the browser and the OS of the device visiting it \cite{phani}, we emulated a diverse set of mobile and desktop devices and different browsers using different browser user agent strings. They are Firefox on Windows, Safari on Mac, Edge on Windows, Chrome on Windows, Chrome on Linux, Chrome on Mac, Chrome on Android Phone,  Safari on iPhone, Safari on iPad, and Chrome on Android Tablets. When a crawler takes a screenshot of the visited webpage, it checks the URL. Suppose the URL's popularity metric on Tranco's list is lower than 10.000. In that case, it randomly changes its viewport three times from a weighted list depending on whether the device is a desktop or mobile device and takes screenshots for different viewports. We used gs.statcounter.com to find the most popular screen resolutions worldwide. Another thing to consider is that the visible area to the user or the viewport of a web browser generally varies by device, even when the devices have the same resolution and screen. We had to consider this while taking screenshots. Because we want the aspect ratios of our screenshots as close to what user sees when they browse the web. To consider this, we analyzed the viewport size of 400 real users using Amazon Mechanical Turk \cite{turk}. With that, we saw the relationship between the actual resolution and viewport size and the existence of different viewports and their popularity by resolution, and we specified a weight per viewport that affects the random picking of that viewport area when taking screenshots. To make the crawling as stealthy as possible and prevent detection of the anti-bot mechanisms implemented by some of the ad networks, we used the stealth libraries of the puppeteer \cite{stealth}. Finally, we utilized Docker to containerize our puppeteer crawlers and ran them on both benign and SE URL lists we gathered. Each crawler within a Docker container visited URLs using a fixed user agent, and all user agent strings were employed for visiting each URL.



\subsubsection{\textbf{Extract Crawling Logs}}
The collected logs mentioned in step 2 have been saved in our server in a compressed manner. When crawling was completed, we created various parser scripts to extract the required data from those logs. Here, we extracted the traceback logs and collected screenshots with the URLs they belong to. 


\subsubsection{\textbf{Dataset Preparation}}

To make the screenshots ready for the deep learning pipeline, we followed the steps below:
\paragraph{\textbf{Duplicate Elimination:}} Our crawler is programmed to take a screenshot of a page before clicking on a coordinate. After the click, it checks if the HTML of the web page has changed. If yes, it takes a screenshot after the click. We take that after-screenshot to see if the clicks trigger any modifications to the page's HTML code for further analysis. Sometimes, that change does not trigger any visual difference, and we collect duplicate screenshots. To eliminate those duplicate screenshots, we used the MD5 hash. We eliminated duplications if we collected them from the same URLs. That way, we did not lose the same SE screenshots reached from different URLs. To make the model training faster and reduce GPU memory and hard disk usage, the quality of the screenshots obtained after is reduced by 10%. At the same time, we converted them into the JPG format without compromising the visual composition of the screenshots. 
\paragraph{\textbf{Resolution Separation:}} We separated the screenshots obtained after step 3 by their resolutions via a script, and the result is 28 different folders containing a total of around 396.000 screenshots for the SE crawlers and 94.000 screenshots for the benign crawlers. The main reason we separate the screenshots by resolution is to facilitate the batch creation of the fully convolutional deep learning model. As we know, every batch created during the model training must contain screenshots from the same dimensions. 
\paragraph{\textbf{Metaclustering:}} We wanted to remove the screenshots unrelated to social engineering attacks from the SE-crawlers collected screenshots. What sets social engineering attacks apart is that even if they come from different domains, their visuality is the same or close to each other to circumvent URL blacklists \cite{phani}. Taking advantage of this characteristic, we grouped visually close screenshots under the same cluster and excluded unrelated screenshots. For this purpose, we used a similar technique to \cite{phani}. We obtained a 16-bit length perceptual hash per screenshot under a resolution. And then compared the perceptual hashes, and if the difference between the hashes per screenshot is less than 40, we cluster them together. We found those parameters and the choice of the algorithm as the best one for our dataset. For filtering, the clusters with fewer than 3 screenshots and clusters containing less than 3 second-level domains are eliminated. After that step, we got close to 4000 screenshots and 30 different SE attack campaigns from 28 different resolutions. To improve on the clusters that might have been missed, we visited them manually to check them because it sometimes clusters screenshots that must be under the same clusters into different clusters  (e.g., screenshots with similar visuality or screenshots with varying colors of the background.). To solve that problem, we manually reviewed the clusters obtained and combined similar clusters in terms of visuality and attack category. After that step, those clusters are called metaclusters. We include the Social Engineering metaclusters from another paper \cite{phani} in our dataset to increase metaclusters' variability both in terms of attack categories and aspect ratios. That addition introduced two new resolutions and 30 more metaclusters to our dataset. 
\paragraph{\textbf{Labeling:}} An important step to train a supervised learning model and obtain the ground truth is labeling the dataset. To identify the type of social engineering tactics (if any) were included in the sites visited by our crawler, we rely on the knowledge of multiple experts to form the definitions of SE attacks and its categories that can be followed for labeling them. To that end, we provided the meta-clusters obtained at the end of the previous step to 3 experts for labeling purposes. After a few iterations of labeling different sets of meta clusters and discussions, all 3 experts agreed on a set of definitions of SE attacks and their categories. Note that each meta-cluster is labelled as a whole, since all screenshots in a meta-cluster belong to a single SE attack campaign. The labels and their definitions are as follows. First, each of the meta clusters are labelled based on the "strength" of the social engineering attack found in the images. They can belong to only one of the following labels:

\textit{\textbf{d.1. Strictly Social Engineering (SSE):}} This label is assigned to those web pages that state an obvious lie to trick users to take unwanted or urgent actions such as installing software, giving permissions, entering their credentials. We can see some examples in Figure 2.

\begin{figure}[ht]
    % \centering
    % \begin{center}
        % \vspace{18pt}%
        % \caption@setup{format=plain,justification=centering}
        \includegraphics[width=9cm,keepaspectratio]{figures/SSE.pdf}
        
        \caption{Examples of SSE campaigns}
    % \end{center}
        
   
    
\end{figure}
\label{fig:SSE}

\textit{\textbf{d.2. Likely Social Engineering (LSE):}} This label is assigned to those web pages with no obvious lie but still contains different indicators to be deemed as Social Engineering Attack. The indicators could be one or more of the following 

  \textit{\textbf{d.2.1. LSE1:}} The design of the images is similar to already seen SE pages (based on previous work and the expert labelers' own experience). In a few cases, since there was no obvious lie to manipulate users, additional evidence may need to be collected by visiting the page manually or looking at the crawling logs to determine if the interaction with the page resulted in a malicious binary download. 
  \begin{figure}[ht]
    % \centering
    \begin{center}
        % \vspace{18pt}%
        % \caption@setup{format=plain,justification=centering}
        \includegraphics[width=9cm,keepaspectratio]{figures/LSE1.pdf}
        
        \caption{Examples of LSE1 campaigns}
    \end{center}
        
   
    
\end{figure}
\label{fig:LSE1}

  \textit{\textbf{d.2.2. LSE2:}} If the main design of the screenshots belonging to the same meta-cluster is the same except there are subtle changes such as different logos were used to provide variability to the attack, or the page contains dynamics elements (such as comments section) or timestamps that should change over time but remain same for different examples visited at different times. 

  \begin{figure}[ht]
    % \centering
    \begin{center}
        % \vspace{18pt}%
        % \caption@setup{format=plain,justification=centering}
        \includegraphics[width=9cm,keepaspectratio]{figures/LSE2.pdf}
        
        \caption{Examples of LSE2 campaigns}
    \end{center}
        
   
    
\end{figure}
\label{fig:LSE2}

\textit{\textbf{d.3. Suspicious:}} This label is assigned to clusters that contain images that do not resemble any of the images we have encountered in the past or in the wild. However, they still try to collect personal information from the user, and they do not belong to the Tranco's most popular 10,000 domains. Further, the page content was also found to be hosted on multiple domains that are unrelated, unlike benign websites. Therefore, we mark these as suspicious.  
\begin{figure}[ht]
    % \centering
    \begin{center}
        % \vspace{18pt}%
        % \caption@setup{format=plain,justification=centering}
        \includegraphics[width=6cm,keepaspectratio]{figures/suspicious.pdf}
        
        \caption{Examples of Suspicious campaigns}
    \end{center}
\end{figure}
\label{fig:suspicious}
\textit{\textbf{d.4. Unknown:}} The labelers cannot determine the nature of the page (whether it contains any suspected threats or it is benign). 

\begin{figure}[ht]
    % \centering
    \begin{center}
        % \vspace{18pt}%
        % \caption@setup{format=plain,justification=centering}
        \includegraphics[width=6cm,keepaspectratio]{figures/unknown.pdf}
        
        \caption{Examples of Unknown campaigns}
    \end{center}
\end{figure}
\label{fig:unknown}

\textit{\textbf{d.5. Benign:}} This label is assigned for the screenshots derived from the benign crawlers. Because we visited the most 5000 popular websites, and all the visited URL the possibility of obtaining a social engineering attack screenshot is extremely low.

After we completed the labeling, 3 experts unanimously decided to use metaclusters labeled SSE, and LSE for training and call its class SE or malicious and use benign labeled screenshots for the benign class. We considered social engineering metaclusters which cover the full page rather than presenting themselves as notifications or just a small part of the page.


\paragraph{\textbf{Data Augmentation:}} To increase the deep learning model's generalization power, we randomly select images to be augmented, which we augment with an augmentation method chosen at random among the ones listed below. This allowed us to increase the size of the dataset to 15.000 benign and 15.000 SE (500 screenshots per resolution). Because of the nature of the webpage content, we made sure not to corrupt either the readability of the text content or the orientation of the webpage object when we chose the augmentation functions. We apply random parameters for the image augmentation functions to reduce the possibility of obtaining duplicate images. Every image undergoes the following image augmentation methods: 

\textit{\textbf{Applying Color inversion:}} We apply it at most once to avoid duplication because there is no randomized parameter. 

\textit{\textbf{Applying Gray Scaling:}} We apply it at most once to avoid duplication because there is no randomized parameter. 

\textit{\textbf{Scaling and Random Cropping:}} We apply it as one operation, images are scaled from random edges, not from the center, between \%10 and \%20, and then We crop them to their original resolution. 

\textit{\textbf{Changing hue:}} We change the hue randomly between -0.5 and +0.5 of the original hue. 

\textit{\textbf{Changing saturation:}} We change the saturation randomly between \%10 and \%250 of the original saturation. 

\textit{\textbf{Changing contrast:}} We change the contrast randomly between \%10 and \%250 of the original contrast. 

\textit{\textbf{Changing brightness:}} We change the brightness randomly between \%10 and \%250 of the original brightness. 

\textit{\textbf{Randomly Solarize:}} We solarize the pixels of the image if their value is above the randomly defined threshold specified between 0 and 255.

\subsubsection{\textbf{Combined Dataset Creation}}
We wanted to create an additional dataset to see if we could get an increase in the detection performance of the model. For this purpose, we used the traceback logs and traced the labeled SE screenshots back to the landing page leading to those attacks. For the benign combined set, we just paired benign screenshots coming from different second-level domains. We followed this path for the benign screenshot because we saw that in almost all cases, the social engineering attacks are hosted on different domains than the publisher landing pages. After that, we concatenated the landing page and attack page pairs side by side and augmented this set for training in the same way we did for the single dataset and called it the combined dataset.



\subsection{\textbf{Deep Learning}}
We employed TensorFlow API's transfer learning models to attain optimal classification performance. Transfer learning enhances training efficiency, diminishes the data requirements for training, and improves performance by leveraging pre-trained deep learning models that were initially trained on the same domain. The datasets created above will be supplied to our custom deep-learning pipeline here. But Before that, We should select one of the available transfer learning models, find the optimal model architecture, implement the custom federated learning, and tune the hyperparameters of the model.

\subsubsection{\textbf{Model Selection}}
Our initial experiments employed the state-of-the-art transfer learning models: Inception-ResNet-v2 \cite{Szegedy}, ResNet50V2 \cite{Kaiming}, VGG-16, VGG-19 \cite{Simonyan}, and Xception \cite{Chollet}. The weights of those models have been trained on the Imagenet Large Scale Visual Recognition Challenge dataset \cite{Imagenet,Imagenetchallenge}. We aimed to find the best model accuracy tradeoff, the lowest false positives, and resource usage. To find the best performant model on our dataset, we compared them on a fixed dataset, disabled all random initializations, and used a deterministic approach \cite{determinism} .After conducting experiments on various models, we found that the VGG-19 model yielded the lowest rates of false positives and false negatives. As a result, we opted to further compare and incorporate that model in our research.

\subsubsection{\textbf{Selected Model Architecture}}
The VGG19 architecture, developed by the Visual Geometry Group at the University of Oxford, represents a deep convolutional neural network (CNN) model comprising 19 layers. This includes 16 convolutional layers and 3 fully connected layers. With a stride of 1, the convolutional layers employ 3x3 filters and are accompanied by rectified linear unit (ReLU) activations. 2x2 max-pooling layers with a stride of 2 are utilized to downsample the feature maps. The fully connected layers are responsible for the final classification stage, typically employing softmax activation for multi-class classification. Widely recognized for its simplicity and depth, VGG19 has exhibited remarkable performance across various computer vision tasks, including image classification and object detection \cite{Simonyan}
\\The VGG-19 network operates on RGB images of a consistent size of 224x224 pixels. As our network was trained on web browsing screenshots obtained emulating various mobile and desktop devices with varying aspect ratios, utilizing a fixed input size may result in distortion and reduced accuracy in detection, mainly when dealing with mobile portrait images. Those images often possess a significantly greater height than their widths, making it crucial to consider this aspect for improved detection performance. To address this issue, we employed the Fully Convolutional Neural Networks(FCNN) architecture. \cite{Jonathan} has demonstrated successful classification capabilities of FCNNs when working with images of diverse sizes.
\\To prepare the VGG-19 model for our pipeline, we loaded the VGG-19 model trained on the Imagenet dataset. Subsequently, We removed the classification head and dense layers. 
\\To convert the model into a Fully Convolutional Network, We included a GlobalMaxPooling2D layer after the last Conv2D layer. This additional layer takes the feature maps produced by the preceding Conv2D layer, identifies the most significant features, and applies max pooling across the entire feature map. As a result, a single value is obtained for each channel in the feature map.
\\Finally, we included a dense layer in our binary classification task, consisting of two neurons and utilizing the Softmax activation function for classification.

\subsubsection{\textbf{Implementation of Federated Learning}}
While conducting training, we obtained approximately 35,000 images from 60 different resolutions after applying data augmentation techniques. However, attempting to train such a large image dataset on a single GPU, specifically the NVIDIA A40 48GB GPU, and the Dell PowerEdge R750xa with 256GB CPU memory, led to memory exhaustion. To overcome this challenge, we devised a customized version of the federated learning approach.
\\Federated learning \cite{McMahan} is a technique in machine learning where numerous devices or entities collaborate to train a shared model without sharing their raw data. Instead, each device performs local training and only shares model updates with a central server. This approach prioritizes data privacy and minimizes data transfer requirements, making it well-suited for domains such as healthcare and finance.

\subsubsection{\textbf{Custom Fully Convolutional Federated Learning Implementation}}
As privacy is not a concern in our specific implementation, the clients and server function as a single entity during training. The algorithm for our Federated Learning approach can be summarized as follows:


\begin{algorithm}
    \caption{Custom Fully Conv. Federated Learning Training}
    \label{alg:ALG1}
    \begin{algorithmic}
    \Require {\\$FVGG19$: FCNN VGG19 model with Imagenet weights\\$GE$: Global epoch count\\$CE$=5: Client epoch count \\$CC$ Client count,\\$SWL$ An empty list to store scaled client weights}
    \Ensure {A trained FCNN VGG19 model}
    \\
    \end{algorithmic}
    \begin{algorithmic}[1]
    \ForAll  {$j=1$ to $GE$}
        \ForAll  {$i=1$ to $CC$}
            \State        Set $clientModel.weights = FVGG19.weights $ 
            \State        Create a dataset for $ith$ client by preprocessing an exact number of images from all resolutions per class
            \State        Train the client model for $CE$ epochs
            \State        Scale the weights of $clientModel$ based on $CC$
            \State        $SWL$.insert($clientModel.weights$)
        \EndFor 
        \State        Set $averageWeights$ = average weights in $SWL$
        \State        Set $FVGG19.weights = averagedClientWeights $ 
        \State        Evaluate $FVGG19$ on validation data
    \EndFor 

    \end{algorithmic}
\end{algorithm}
% \begin{enumerate}

%     \item Initialize the Global VGG-19 model according to the explained architecture.	                   
%     \item Create a client model and transfer the weights from the Global VGG-19 model to it. 
%     \item Load and preprocess images specific to each client, creating a dataset for that client.
%     \item Train the client model for 5 epochs using the client's dataset from step 3.
%     \item Adjust the model's weights by scaling them based on the number of clients present in the model. 
%     \item Store the client model's weight in a list. 
%     \item Repeat steps 2-6 for all clients specified as parameters. 
%     \item Calculate the average of all client model weights stored in the list from Step 5. 
%     \item Transfer the average weight obtained in Step 8 back to the Global Model. 
%     \item Evaluate the Global Model on validation data. 
%     \item For every epoch, Repeat steps 2 to 10. 
% \end{enumerate}
This implementation trains one client at a time using its specific data, which prevents resource exhaustion and provides the benefit of averaging the entire models along with their learned representations. In scenarios involving larger datasets or GPUs/CPUs with limited memory, we can adjust the number of clients to avoid overburdening the resources.

\subsubsection{\textbf{TensorFlow Federated Simulation}}
Initially, we attempted to utilize the pre-existing Federated Simulation environment provided by the TensorFlow library (accessible at \cite{simulation}) before exploring our custom approach. However, during experimentation, we encountered a limitation in the simulation environment. The framework loads the entire preprocessed client datasets into GPU memory just before training begins, leading to GPU memory exhaustion.

\subsubsection{\textbf{Hyperparameter Tuning}}
In that section, we will explain the combination of hyperparameters that results in the best performance of our model on our dataset. We performed those experiments using the same fixed dataset on the same objective and ran all the models deterministically. 
\\We began by freezing the entire network and only training the added layers. Later, we unfroze selected convolutional layers and fine-tuned the network for a few epochs. Fine-tuning plays a crucial role in transfer learning, allowing a pre-trained model to be adjusted for a new task or domain. Typically, a CNN's shallow layers capture fundamental relevant image features across various image analysis tasks. Conversely, the deeper layers focus on extracting application-specific semantic features. Consequently, it is generally enough to fine-tune the final layers for effective transfer learning. As reported in \cite{Tajbakhsh}, in situations involving a scarcity of training data, appropriate fine-tuning exhibited either better or, at the very least, similar performance compared to training a CNN from the start. At the beginning, we initiated training using a learning rate of 0.001 and tested lower and higher learning rates. Concurrently, we unfroze either all or a subset of the 4 block5 and 4 block4 convolutional layers. Through experimentation, we discovered that setting the learning rate to 0.00001 and unfreezing all block5 convolutional layers yielded the best outcomes for our FCNN VGG-19. 
\\As an optimizer, we used Adam after comparing the results with Nadam. 
\\We performed some tests adding a convolutional layer before the GlobalMaxPooling2D. We introduced a 2D Convolutional layer of 128 filters with a stride of 1, rectified linear unit (ReLU) activation, and employed the same padding. The objective of this layer is to reduce the 512 feature maps of various sizes derived from the "block5" of the Fully convolutional VGG-19. \cite{Shuicheng} showed that those 1x1 convolutions introduce additional non-linearity into the network, resulting in a decrease in computational workload while also enhancing the model's ability to acquire more robust representations and it is referred to as "Network in Network". Even though in VGG-19, we could not see any increase in the detection performance, the results were slightly better in Inception-ResNet-v2, ResNet50V2, VGG-16, and Xception models. During those tests, we also tuned the number of filters, starting with 16 and doubling it until 256, and then, we stacked up 2 and 3 convolutional layers. We found that 1 Conv2D layer with 128 filters worked well for all models except the VGG19.

\subsubsection{\textbf{Tuning Other Parameters}}
We tuned various other parameters in the model to increase the detection rate. We used the same fixed dataset for those experiments and trained the models deterministically. When we supplied images to our model during training, we rescaled their width and height by factor 4. We also performed experiments on scaling factors 2,6, and 8. We discovered that scaling factor 4 for the desktop images and scaling factor 2 for the mobile images is the perfect balance between training time and the detection performance of the model.
\\We tested different imaging libraries, specifically TensorFlow and OpenCV libraries, to load and preprocess the images during training and testing. After running the same tasks for both models, we saw that using TensorFlow operations yielded better results, and we used TensorFlow imaging operations for all the experiments.
\\We adjusted the training epochs and the number of clients in our experiment. We tested different numbers of epochs for each client, specifically 1, 3, 5, and 10. Our results showed that 5 epochs with 5 clients worked well for our objective.
\\ \cite{Micikevicius} showed that using half-precision 16-bit floating numbers for the less critical computations and using  32-bit precision floating numbers for critical computations while training a neural network reduces the memory usage and maintains the detection performance and shortens the time required to train a neural network. We performed some experiments using that mixed precision approach and got a similar performance with less training time. However, we decided not to use it because training performed with scaling factor 4 already yielded good performance in our objective.
\\We wanted to test different transfer learning models to achieve the best detection performance and pick the optimal one for our objective. We used different state-of-the-art transfer learning models and compared their results for that purpose. After intensively fine-tuning the hyperparameters we discussed above for the Inception-ResNet-v2, ResNet50V2, VGG-16, VGG-19, and Xception models, VGG-19 performed slightly better on our dataset, and we decided to use that in our paper.



\subsection{\textbf{Research Questions}}
\label{sec:research_questions}
\karthika{We can move this to a different section later.}
